Chasing diagrams in cryptography

Cryptography is a theory of secret functions. Category theory is a general theory of functions. Cryptography has reached a stage where its structures often take several pages to define, and its formulas sometimes run from page to page. Category theory has some complicated definitions as well, but one of its specialties is taming the flood of structure. Cryptography seems to be in need of high level methods, whereas category theory always needs concrete applications. So why is there no categorical cryptography? One reason may be that the foundations of modern cryptography are built from probabilistic polynomial-time Turing machines, and category theory does not have a good handle on such things. On the other hand, such foundational problems might be the very reason why cryptographic constructions often resemble low level machine programming. I present some preliminary explorations towards categorical cryptography. It turns out that some of the main security concepts are easily characterized through the categorical technique of *diagram chasing*, which was first used Lambek's seminal `Lecture Notes on Rings and Modules'.

==> AA-JPEGS/DH-attack.tex <==
%%Created by jPicEdt 1.4.1: mixed JPIC-XML/LaTeX format
%%Fri Nov 14 19:53:23 GMT 2008
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="110" y-min="12.5" y-max="80" auto-bounding="true">
%<parallelogram stroke-width= "0.2"
%	 p3= "(15,12.5)"
%	 p1= "(0,80)"
%	 fill-style= "none"
%	 p2= "(15,80)"
%	 stroke-color= "#666666"
%	 />
%<parallelogram stroke-width= "0.2"
%	 p3= "(65,12.5)"
%	 p1= "(45,80)"
%	 fill-style= "none"
%	 p2= "(65,80)"
%	 stroke-color= "#666666"
%	 />
%<parallelogram stroke-width= "0.2"
%	 p3= "(110,12.5)"
%	 p1= "(95,80)"
%	 fill-style= "none"
%	 p2= "(110,80)"
%	 stroke-color= "#666666"
%	 />
%<multicurve arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 points= "(7.5,60);(7.5,60);(55,60);(55,60)"
%	 />
%<multicurve arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 points= "(55,50);(55,50);(102.5,50);(102.5,50)"
%	 />
%<multicurve arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 points= "(102.5,40);(102.5,40);(55,40);(55,40)"
%	 />
%<multicurve polydots-size-linewidth-scale= "2.5"
%	 right-arrow= "head"
%	 stroke-overstrike-width= "0.75"
%	 polydots-size-minimum= "0.7"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-length-scale= "1.55"
%	 points= "(55,30);(55,30);(7.5,30);(7.5,30)"
%	 polydots-scale-v= "1"
%	 arrow-head-width-minimum= "1.45"
%	 polydots-angle= "0"
%	 fill-style= "none"
%	 polydots-superimpose= "true"
%	 stroke-overstrike= "true"
%	 polydots-scale-h= "1"
%	 polydots-style= "polydots-square"
%	 />
%<multicurve polydots-scale-v= "1"
%	 polydots-size-linewidth-scale= "2.5"
%	 polydots-angle= "0"
%	 fill-style= "none"
%	 polydots-superimpose= "true"
%	 polydots-size-minimum= "0.7"
%	 polydots-scale-h= "1"
%	 polydots-style= "polydots-square"
%	 points= "(7.5,70);(7.5,70);(7.5,60);(7.5,60)"
%	 />
%<multicurve polydots-scale-v= "1"
%	 polydots-size-linewidth-scale= "2.5"
%	 polydots-angle= "0"
%	 fill-style= "none"
%	 polydots-superimpose= "true"
%	 polydots-size-minimum= "0.7"
%	 polydots-scale-h= "1"
%	 polydots-style= "polydots-square"
%	 points= "(55,60);(55,60);(55,50);(55,50)"
%	 />
%<multicurve polydots-scale-v= "1"
%	 polydots-size-linewidth-scale= "2.5"
%	 polydots-angle= "0"
%	 fill-style= "none"
%	 polydots-superimpose= "true"
%	 polydots-size-minimum= "0.7"
%	 polydots-scale-h= "1"
%	 polydots-style= "polydots-square"
%	 points= "(102.5,50);(102.5,50);(102.5,40);(102.5,40)"
%	 />
%<multicurve polydots-scale-v= "1"
%	 polydots-size-linewidth-scale= "2.5"
%	 polydots-angle= "0"
%	 fill-style= "none"
%	 polydots-superimpose= "true"
%	 polydots-size-minimum= "0.7"
%	 polydots-scale-h= "1"
%	 polydots-style= "polydots-square"
%	 points= "(55,40);(55,40);(55,30);(55,30)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(2.5,77.5)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\alice$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(47.5,77.5)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\eve$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(97.5,77.5)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\bob$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(6.25,65)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\newa$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(103.75,45)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\newb$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(20,60.62)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\msgOne$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(70.62,40.62)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\msgTwoBack$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,32.5)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\msgOneBack$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(22.5,62.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(80,50.62)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\msgTwo$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(54.38,55)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\newmTwo$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(55.62,35)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\newmOne$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(7.5,15)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\keyAB$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(102.5,15)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\keyBA$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(46,15)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\keyAM$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(64,15)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\keyMB$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(110,80)
\newrgbcolor{userLineColour}{0.4 0.4 0.4}
\pspolygon[linewidth=0.2,linecolor=userLineColour](0,80)(15,80)(15,12.5)(0,12.5)
\newrgbcolor{userLineColour}{0.4 0.4 0.4}
\pspolygon[linewidth=0.2,linecolor=userLineColour](45,80)(65,80)(65,12.5)(45,12.5)
\newrgbcolor{userLineColour}{0.4 0.4 0.4}
\pspolygon[linewidth=0.2,linecolor=userLineColour](95,80)(110,80)(110,12.5)(95,12.5)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(7.5,60)(55,60)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(55,50)(102.5,50)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(102.5,40)(55,40)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(55,30)(7.5,30)
\psdots[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55,dotstyle=square](55,30)
(7.5,30)
\psline(7.5,70)(7.5,60)
\psdots[dotstyle=square](7.5,70)
(7.5,60)
\psline(55,60)(55,50)
\psdots[dotstyle=square](55,60)
(55,50)
\psline(102.5,50)(102.5,40)
\psdots[dotstyle=square](102.5,50)
(102.5,40)
\psline(55,40)(55,30)
\psdots[dotstyle=square](55,40)
(55,30)
\rput[l](2.5,77.5){$\alice$}
\rput[l](47.5,77.5){$\eve$}
\rput[l](97.5,77.5){$\bob$}
\rput[r](6.25,65){$\newa$}
\rput[l](103.75,45){$\newb$}
\rput[bl](20,60.62){$\msgOne$}
\rput[bl](70.62,40.62){$\msgTwoBack$}
\rput[l](20,32.5){$\msgOneBack$}
\rput[b](22.5,62.5){}
\rput[b](80,50.62){$\msgTwo$}
\rput[r](54.38,55){$\newmTwo$}
\rput[l](55.62,35){$\newmOne$}
\rput(7.5,15){$\keyAB$}
\rput(102.5,15){$\keyBA$}
\rput[l](46,15){$\keyAM$}
\rput[r](64,15){$\keyMB$}
\end{pspicture}


==> AA-JPEGS/DHKA.tex <==
%%Created by jPicEdt 1.4.1: mixed JPIC-XML/LaTeX format
%%Fri Nov 14 19:54:28 GMT 2008
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="110" y-min="12.5" y-max="80" auto-bounding="true">
%<parallelogram stroke-width= "0.2"
%	 p3= "(15,12.5)"
%	 p1= "(0,80)"
%	 fill-style= "none"
%	 p2= "(15,80)"
%	 stroke-color= "#666666"
%	 />
%<parallelogram stroke-width= "0.2"
%	 p3= "(110,12.5)"
%	 p1= "(95,80)"
%	 fill-style= "none"
%	 p2= "(110,80)"
%	 stroke-color= "#666666"
%	 />
%<multicurve arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 points= "(7.5,55);(7.5,55);(102.5,55);(102.5,55)"
%	 />
%<multicurve polydots-size-linewidth-scale= "2.5"
%	 right-arrow= "head"
%	 stroke-overstrike-width= "0.75"
%	 polydots-size-minimum= "0.7"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-length-scale= "1.55"
%	 points= "(102.5,35);(102.5,35);(7.5,35);(7.5,35)"
%	 polydots-scale-v= "1"
%	 arrow-head-width-minimum= "1.45"
%	 polydots-angle= "0"
%	 fill-style= "none"
%	 polydots-superimpose= "true"
%	 stroke-overstrike= "true"
%	 polydots-scale-h= "1"
%	 polydots-style= "polydots-square"
%	 />
%<multicurve polydots-scale-v= "1"
%	 polydots-size-linewidth-scale= "2.5"
%	 polydots-angle= "0"
%	 fill-style= "none"
%	 polydots-superimpose= "true"
%	 polydots-size-minimum= "0.7"
%	 polydots-scale-h= "1"
%	 polydots-style= "polydots-square"
%	 points= "(7.5,70);(7.5,70);(7.5,55);(7.5,55)"
%	 />
%<multicurve polydots-scale-v= "1"
%	 polydots-size-linewidth-scale= "2.5"
%	 polydots-angle= "0"
%	 fill-style= "none"
%	 polydots-superimpose= "true"
%	 polydots-size-minimum= "0.7"
%	 polydots-scale-h= "1"
%	 polydots-style= "polydots-square"
%	 points= "(102.5,55);(102.5,55);(102.5,35);(102.5,35)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(2.5,77.5)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\alice$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(97.5,77.5)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\bob$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(6.25,65)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\newa$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(103.75,45)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\newb$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(45,55.62)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\msgOne$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(45.62,35.62)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\msgOneBack$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(22.5,62.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(7.5,15)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\keyAB$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(102.5,15)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\keyBA$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(45,54.38)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\intoOne$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(45.62,34.38)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\intoOneBack$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(110,80)
\newrgbcolor{userLineColour}{0.4 0.4 0.4}
\pspolygon[linewidth=0.2,linecolor=userLineColour](0,80)(15,80)(15,12.5)(0,12.5)
\newrgbcolor{userLineColour}{0.4 0.4 0.4}
\pspolygon[linewidth=0.2,linecolor=userLineColour](95,80)(110,80)(110,12.5)(95,12.5)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(7.5,55)(102.5,55)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(102.5,35)(7.5,35)
\psdots[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55,dotstyle=square](102.5,35)
(7.5,35)
\psline(7.5,70)(7.5,55)
\psdots[dotstyle=square](7.5,70)
(7.5,55)
\psline(102.5,55)(102.5,35)
\psdots[dotstyle=square](102.5,55)
(102.5,35)
\rput[l](2.5,77.5){$\alice$}
\rput[l](97.5,77.5){$\bob$}
\rput[r](6.25,65){$\newa$}
\rput[l](103.75,45){$\newb$}
\rput[bl](45,55.62){$\msgOne$}
\rput[bl](45.62,35.62){$\msgOneBack$}
\rput[b](22.5,62.5){}
\rput(7.5,15){$\keyAB$}
\rput(102.5,15){$\keyBA$}
\rput[tl](45,54.38){$\intoOne$}
\rput[tl](45.62,34.38){$\intoOneBack$}
\end{pspicture}


==> AA-JPEGS/SSec-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Dec 03 13:35:20 PST 2009
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="151.62" y-min="-1.25" y-max="43.75" auto-bounding="true">
%<multicurve arrow-head-length-scale= "1.55"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-width-minimum= "1.45"
%	 fill-style= "none"
%	 points= "(5,41);(5,41);(21,41);(21,41)"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-width-minimum= "1.45"
%	 fill-style= "none"
%	 points= "(7,0);(7,0);(142.5,0);(142.5,0)"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-width-minimum= "1.45"
%	 fill-style= "none"
%	 points= "(150.62,37.25);(150.62,37.25);(150.62,6.25);(150.62,6.25)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(0,41)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\ulid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(32,41)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\urid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(0,0)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\dlid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(151.25,0)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\drid$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(11.88,41.88)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\upid$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(75,-1.25)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\downid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(151.62,21.25)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\rightid$
%</text>
%<multicurve arrow-head-length-scale= "1.55"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-width-minimum= "1.45"
%	 fill-style= "none"
%	 points= "(46,41);(46,41);(76,41);(76,41)"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-width-minimum= "1.45"
%	 fill-style= "none"
%	 points= "(120,41);(120,41);(138,41);(138,41)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(96.88,41.25)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\urrid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(150,41.25)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\urrrid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,43.75)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\uppid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(127.5,43.75)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\upppid$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(151.62,43.75)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(5,41)(21,41)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(7,0)(142.5,0)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(150.62,37.25)(150.62,6.25)
\rput(0,41){$\ulid$}
\rput(32,41){$\urid$}
\rput(0,0){$\dlid$}
\rput(151.25,0){$\drid$}
\rput[b](11.88,41.88){$\upid$}
\rput[t](75,-1.25){$\downid$}
\rput[l](151.62,21.25){$\rightid$}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(46,41)(76,41)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(120,41)(138,41)
\rput(96.88,41.25){$\urrid$}
\rput(150,41.25){$\urrrid$}
\rput(60,43.75){$\uppid$}
\rput(127.5,43.75){$\upppid$}
\end{pspicture}


==> AA-JPEGS/SSec.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Dec 03 13:26:58 PST 2009
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-1" x-max="151.62" y-min="-1.25" y-max="43.75" auto-bounding="true">
%<multicurve arrow-head-length-scale= "1.55"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-width-minimum= "1.45"
%	 fill-style= "none"
%	 points= "(5,41);(5,41);(21,41);(21,41)"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-width-minimum= "1.45"
%	 fill-style= "none"
%	 points= "(7,0);(7,0);(142.5,0);(142.5,0)"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-width-minimum= "1.45"
%	 fill-style= "none"
%	 points= "(0,36.25);(0,36.25);(0,5);(0,5)"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-width-minimum= "1.45"
%	 fill-style= "none"
%	 points= "(150.62,37.25);(150.62,37.25);(150.62,6.25);(150.62,6.25)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(0,41)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\ulid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(32,41)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\urid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(0,0)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\dlid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(151.25,0)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\drid$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(11.88,41.88)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\upid$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(75,-1.25)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\downid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(-1,20)"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\leftid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(151.62,21.25)"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\rightid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(76.88,20)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\eqls$
%</text>
%<multicurve arrow-head-length-scale= "1.55"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-width-minimum= "1.45"
%	 fill-style= "none"
%	 points= "(46,41);(46,41);(76,41);(76,41)"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 stroke-overstrike-width= "0.75"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-width-minimum= "1.45"
%	 fill-style= "none"
%	 points= "(120,41);(120,41);(138,41);(138,41)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(96.88,41.25)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\urrid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(150,41.25)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\urrrid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,43.75)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\uppid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(127.5,43.75)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$\upppid$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(151.62,43.75)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(5,41)(21,41)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(7,0)(142.5,0)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(0,36.25)(0,5)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(150.62,37.25)(150.62,6.25)
\rput(0,41){$\ulid$}
\rput(32,41){$\urid$}
\rput(0,0){$\dlid$}
\rput(151.25,0){$\drid$}
\rput[b](11.88,41.88){$\upid$}
\rput[t](75,-1.25){$\downid$}
\rput[r](-1,20){$\leftid$}
\rput[l](151.62,21.25){$\rightid$}
\rput(76.88,20){$\eqls$}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(46,41)(76,41)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(120,41)(138,41)
\rput(96.88,41.25){$\urrid$}
\rput(150,41.25){$\urrrid$}
\rput(60,43.75){$\uppid$}
\rput(127.5,43.75){$\upppid$}
\end{pspicture}


==> AA-JPEGS/Vcat.tex <==
%%Created by jPicEdt 1.4.1: mixed JPIC-XML/LaTeX format
%%Wed Apr 01 00:53:57 PDT 2009
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="18.75" x-max="150.62" y-min="8.75" y-max="62.5" auto-bounding="true">
%<multicurve arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-length-scale= "1.55"
%	 points= "(40,40);(40,40);(65,40);(65,40)"
%	 />
%<text text-vert-align= "bottom"
%	 anchor-point= "(22.5,62.5)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%
%</text>
%<multicurve arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-length-scale= "1.55"
%	 points= "(35,10);(35,10);(70,10);(70,10)"
%	 />
%<multicurve arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-length-scale= "1.55"
%	 points= "(20,35);(20,35);(20,15);(20,15)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,40)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\ul$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(80,40)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\ur$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,10)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\dl$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(80,10)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\dr$
%</text>
%<multicurve arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-length-scale= "1.55"
%	 points= "(80,35);(80,35);(80,15);(80,15)"
%	 />
%<multicurve arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-length-scale= "1.55"
%	 points= "(115,40);(115,40);(140,40);(140,40)"
%	 />
%<multicurve arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-length-scale= "1.55"
%	 points= "(110,10);(110,10);(145,10);(145,10)"
%	 />
%<multicurve arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-length-scale= "1.55"
%	 points= "(100,35);(100,35);(100,15);(100,15)"
%	 />
%<multicurve arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-length-scale= "1.55"
%	 points= "(150,35);(150,35);(150,15);(150,15)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(100,40)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\ulid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(150,40)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\urid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(100,10)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\dlid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(150,10)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\drid$
%</text>
%<multicurve arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-length-scale= "1.55"
%	 points= "(105.62,35.62);(105.62,35.62);(145,13.75);(145,13.75)"
%	 />
%<text text-vert-align= "bottom"
%	 anchor-point= "(50,41.25)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\up$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(50,8.75)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\down$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(130,40.62)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\upid$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(130,8.75)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\downid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(98.75,25)"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 >
%$\leftid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(150.62,25)"
%	 fill-style= "none"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 >
%$\rightid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(18.75,25)"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 >
%$\leftt$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(81.25,25)"
%	 fill-style= "none"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 >
%$\rightt$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(150.62,62.5)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(40,40)(65,40)
\rput[b](22.5,62.5){}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(35,10)(70,10)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(20,35)(20,15)
\rput(20,40){$\ul$}
\rput(80,40){$\ur$}
\rput(20,10){$\dl$}
\rput(80,10){$\dr$}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(80,35)(80,15)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(115,40)(140,40)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(110,10)(145,10)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(100,35)(100,15)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(150,35)(150,15)
\rput(100,40){$\ulid$}
\rput(150,40){$\urid$}
\rput(100,10){$\dlid$}
\rput(150,10){$\drid$}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(105.62,35.62)(145,13.75)
\rput[b](50,41.25){$\up$}
\rput[t](50,8.75){$\down$}
\rput[b](130,40.62){$\upid$}
\rput[t](130,8.75){$\downid$}
\rput[r](98.75,25){$\leftid$}
\rput[l](150.62,25){$\rightid$}
\rput[r](18.75,25){$\leftt$}
\rput[l](81.25,25){$\rightt$}
\end{pspicture}


==> AA-JPEGS/Vdep.tex <==
%%Created by jPicEdt 1.4.1: mixed JPIC-XML/LaTeX format
%%Wed Apr 01 01:52:52 PDT 2009
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="8.75" x-max="95.62" y-min="3.75" y-max="86" auto-bounding="true">
%<multicurve arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-length-scale= "1.55"
%	 points= "(42,85);(42,85);(63,85);(63,85)"
%	 />
%<text text-vert-align= "bottom"
%	 anchor-point= "(21.88,67.5)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%
%</text>
%<multicurve arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-length-scale= "1.55"
%	 points= "(35,55);(35,55);(70,55);(70,55)"
%	 />
%<multicurve arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-length-scale= "1.55"
%	 points= "(20,80);(20,80);(20,60);(20,60)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,85)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\ul$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(80,85)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\ur$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,55)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\dl$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(80,55)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\dr$
%</text>
%<multicurve arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-length-scale= "1.55"
%	 points= "(80,80);(80,80);(80,60);(80,60)"
%	 />
%<multicurve arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-length-scale= "1.55"
%	 points= "(55,35);(55,35);(80,35);(80,35)"
%	 />
%<multicurve arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-length-scale= "1.55"
%	 points= "(95,30);(95,30);(95,10);(95,10)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(45,35)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\ulid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(95,35)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\urid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(95,5)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\drid$
%</text>
%<multicurve arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-length-scale= "1.55"
%	 points= "(50.62,30.62);(50.62,30.62);(90,8.75);(90,8.75)"
%	 />
%<text text-vert-align= "bottom"
%	 anchor-point= "(52,86)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\up$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(50,53.75)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\down$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(66.88,35.62)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\upid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(95.62,20)"
%	 fill-style= "none"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 >
%$\rightid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(18.75,70)"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 >
%$\leftt$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(81.25,70)"
%	 fill-style= "none"
%	 text-hor-align= "left"
%	 text-frame= "noframe"
%	 >
%$\rightt$
%</text>
%<multicurve arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-length-scale= "1.55"
%	 points= "(22.5,5);(22.5,5);(53.12,5);(53.12,5)"
%	 />
%<multicurve arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-length-scale= "1.55"
%	 points= "(10,30);(10,30);(10,10);(10,10)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,35)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\ulid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,5)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\dlid$
%</text>
%<multicurve arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 stroke-overstrike= "true"
%	 right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-length-scale= "1.55"
%	 points= "(15.62,30.62);(15.62,30.62);(55,8.75);(55,8.75)"
%	 />
%<text text-vert-align= "top"
%	 anchor-point= "(38.12,3.75)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\downid$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(8.75,20)"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 text-frame= "noframe"
%	 >
%$\leftid$
%</text>
%<text text-rotation= "-30"
%	 text-vert-align= "bottom"
%	 anchor-point= "(35,21)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\idd$
%</text>
%<text text-rotation= "-30"
%	 text-vert-align= "top"
%	 anchor-point= "(65.62,21.25)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\ddiag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(60.62,5)"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\ulid$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(95.62,86)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(42,85)(63,85)
\rput[b](21.88,67.5){}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(35,55)(70,55)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(20,80)(20,60)
\rput(20,85){$\ul$}
\rput(80,85){$\ur$}
\rput(20,55){$\dl$}
\rput(80,55){$\dr$}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(80,80)(80,60)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(55,35)(80,35)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(95,30)(95,10)
\rput(45,35){$\ulid$}
\rput(95,35){$\urid$}
\rput(95,5){$\drid$}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(50.62,30.62)(90,8.75)
\rput[b](52,86){$\up$}
\rput[t](50,53.75){$\down$}
\rput[b](66.88,35.62){$\upid$}
\rput[l](95.62,20){$\rightid$}
\rput[r](18.75,70){$\leftt$}
\rput[l](81.25,70){$\rightt$}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(22.5,5)(53.12,5)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(10,30)(10,10)
\rput(10,35){$\ulid$}
\rput(10,5){$\dlid$}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(15.62,30.62)(55,8.75)
\rput[t](38.12,3.75){$\downid$}
\rput[r](8.75,20){$\leftid$}
\rput[b]{-30}(35,21){$\idd$}
\rput[t]{-30}(65.62,21.25){$\ddiag$}
\rput(60.62,5){$\ulid$}
\end{pspicture}

